Deep Multi-Fidelity Active Learning of High-dimensional Outputs

Many applications, such as in physical simulation and engineering design, demand we estimate functions with high-dimensional outputs. The training examples can be collected with different fidelities to allow a cost/accuracy trade-off. In this paper, we consider the active learning task that identifies both the fidelity and input to query new training examples so as to achieve the best benefit-cost ratio. To this end, we propose DMFAL, a Deep Multi-Fidelity Active Learning approach. We first develop a deep neural network-based multi-fidelity model for learning with high-dimensional outputs, which can flexibly, efficiently capture all kinds of complex relationships across the outputs and fidelities to improve prediction. We then propose a mutual information-based acquisition function that extends the predictive entropy principle. To overcome the computational challenges caused by large output dimensions, we use multi-variate Delta's method and moment-matching to estimate the output posterior, and Weinstein-Aronszajn identity to calculate and optimize the acquisition function. The computation is tractable, reliable and efficient. We show the advantage of our method in several applications of computational physics and engineering design.

==> exp_zhe.tex <==
%\vspace{-0.15in}
\section{Experiment}
%\vspace{-0.05in}
\subsection{Solving Partial Differential Equations}
%\vspace{-0.05in}
\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{ccc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/rmse_Burgers.pdf}
			\caption{Burgers' equation}
		\end{subfigure} &
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/rmse_Heat2.pdf}
			\caption{Heat equation}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/rmse_Poisson2.pdf}
			\caption{Poisson's equation}
		\end{subfigure}
	\end{tabular}
%	\vspace{-0.1in}
	\caption{\small Normalized root-mean-square error (nRMSE) for active learning of PDE solution fields with two-fidelity queries. The normalizer is the mean of the test outputs. The results are averaged from five runs. The shaded regions indicate the standard deviations.} \label{fig:solving-pde-2fid}
%	\vspace{-0.2in}
\end{figure*}
We first evaluated \ours in standard computational physics tasks. Specifically, we used \ours to predict the solution fields of  three commonly used partial differential equations (PDEs): \textit{Burgers}'s , \textit{Poisson}'s and \textit{Heat} equations~\citep{olsen2011numerical}. The training examples are collected by running a numerical solver with different meshes. The more the nodes/steps to create the mesh, the higher the fidelity. The input includes the PDE parameters and/or parameterized initial or boundary conditions. The output consists of the solution values at the mesh used in the solver. For example, a $50 \times 50$ mesh corresponds to a $2,500$ dimensional output vector.  To perform active learning, we considered two-fidelity queries for all the three equations, where the sizes of the corresponding output fields are $16 \times 16$ and $32 \times 32$. In addition, we considered a three-fidelity setting for Poisson's equation, denoted by Poisson-3, and the sizes of the output fields of the three fidelities are $16 \times 16$ , $32 \times 32$, and $64 \times 64$, respectively. For the two-fidelity active learning, we uniformly sampled the inputs, and queried $10$ training examples at the first fidelity and $2$ at the second fidelity. We used those examples as the initial training dataset. Similarly, for Poisson-3, we collected $10$, $5$ and $2$ examples in the first, second, and third fidelity as the initial training set. We generated $500$ samples for test, where the test inputs were uniformly sampled from the domain. The outputs are calculated by running the solver with an even denser mesh --- $128 \times 128$ for Burger's and Poisson's equations, and $100 \times 100$ for Heat equation --- and interpolating the solution values at the target grid~\citep{zienkiewicz1977finite} (this is the standard approach in physical simulation and  the accuracy does not change). More details are given in the supplementary material. We ran the solvers at each fidelity for many times and calculated the average running time. We then normalized the average running time to obtain $\lambda_1 = 1$, $\lambda_2 = 3$ and $\lambda_3 = 10$. 

\noindent\textbf{Competing methods.}  We compared \ours with the following active learning approaches. (1) \texttt{MF-BALD},   a straightforward extension of BALD~\citep{houlsby2011bayesian} to integrate multi-fidelity queries. The acquisition function is 
\begin{align}
&a_{\text{MF-BALD}}(\x, m) = \frac{1}{\lambda_m} \mathbb{I}\big(\y_m(\x), \Wcal|\Dcal\big) =\frac{1}{\lambda_m}\left(\mathbb{H}(\y_m(\x)|\Dcal) - \EE_{p(\Wcal|\Dcal)}\left[\mathbb{H}(\y_m(\x)|\Wcal, \Dcal)\right]\right) \notag \\
&=\frac{1}{\lambda_m}\left(\mathbb{H}(\y_m(\x)|\Dcal) - \frac{d_m}{2}\log(2\pi e \sigma_m^2)\right). \label{eq:mf-bald}
\end{align}
Note that conditioned the NN parameters, the entropy of the observed output $\y_m$ is only determined by the noise variance $\sigma_m^2$.  
 (2) \texttt{Dropout-latent}, where we use MC dropout~\citep{gal2017deep} for variational inference, each time draw $100$ dropout samples for the low dimensional latent outputs $\{\f_1(\x), \ldots, \f_M(\x)\}$ to estimate multi-variate Gaussian posteriors for each $\f_m$ and $\barf_m = [\f_m; \f_M]$ (via empirical means and covariance matrices), and then follow Section \ref{sect:ac-compute} to calculate and optimize the acquisition function \eqref{eq:ac}. Note that we have also used MC dropout to outright sample the final, high-dimensional outputs $\{\y_m\}$ and estimate multi-variate Gaussian posteriors to calculate \eqref{eq:ac} and \eqref{eq:mf-bald}. While doing this is much more expensive, the performance did not improve. Instead, it was way worse than \texttt{Dropout-latent} and \texttt{MF-BALD}. See the details in the supplementary material. (3) \texttt{MF-Random}, where each time we randomly select a fidelity and then an input  to query. 
(4) \texttt{Random-F1}, (5) \texttt{Random-F2}, and (6) \texttt{Random-F3}, where we stick to the first, second and third fidelity, respectively, and randomly sample an input to query each time. \zsdc{(7)  \texttt{Random-partial}, where we randomly select a fidelity $m$, and then optimize \eqref{eq:ac} with $m$ fixed.} 

\begin{figure}
	%\vspace{-0.15in}
	\centering
	%\setlength\tabcolsep{0.01pt}
	\includegraphics[width=0.48\textwidth]{./figs/rmse_Poisson3.pdf}
	%\vspace{-0.3in}
	\caption{\small Normalized root-mean-square error (nRMSE) for active learning of the solution field of Poisson's equation, with three-fidelity queries. The results are averaged from five runs. }
	\label{fig:solving-po-3fid}
	%\vspace{-0.2in}
\end{figure}
\noindent\textbf{Settings and results.} We introduced a two-layer NN for each fidelity and used \texttt{tanh} as the activation function. The layer width  was chosen from $\{8, 16, 32, 64, 128\}$.  We set the same dimension for the latent output in each fidelity and selected it from $\{5, 10, 15, 20\}$. For \texttt{Dropout-latent}, we tuned the dropout rate from $\{0.1, 0.2, 0.3, 0.4, 0.5\}$. All the methods were implemented with PyTorch~\citep{paszke2019pytorch}. We used ADAM~\citep{kingma2014adam} for stochastic optimization, where the learning rate was tuned from $\{10^{-4}, 5 \times 10^{-4}, 10^{-3}, 5 \times 10^{-3}, 10^{-2}\}$.  We set the number of epochs to $2,000$, which is enough for convergence. We conducted five runs for each method, and in each run, we queried $100$ examples. We report the average normalized root-mean-square-error (nRMSE) \textit{vs.} the accumulated cost in Fig.  \ref{fig:solving-pde-2fid} and \ref{fig:solving-po-3fid}. The shaded region shows the standard deviation. We can see that at the beginning, all the methods have the same or comparable performance. Along with more queries, \ours quickly achieves better prediction accuracy, and continues to outperform all the other methods  by a large margin. Therefore, \ours can perform much better with the same cost or achieve the same performance with the smallest cost. It is interesting to see that in Fig. \ref{fig:solving-pde-2fid}a, while all the competing approaches have saturated early, \ours keeps improving its prediction accuracy.
 \texttt{Dropout-latent} and \texttt{MF-BALD} consistently outperform random querying strategies, demonstrating the effectiveness of the information-based acquisition functions. However, \texttt{MF-BALD} only computes the predictive entropy in each single fidelity (plus the entropy of the noise, see \eqref{eq:mf-bald}), and does not consider how the low-fidelity training examples influence the final predictions (\ie at the highest fidelity). Its inferior performance to \ours indicates that a straightforward extension to the original BALD can be suboptimal. The worse performance of \texttt{Dropout-latent} than \ours implies that our structural variational inference can give a better posterior estimation for the latent outputs than the stochastic estimations constructed from the dropout samples. Overall,  these results have demonstrated the advantage of our deep multi-fidelity active learning  approach. 
%\vspace{-0.2in}
\subsection{Topology Structure Optimization}
%\vspace{-0.05in}
Next, we applied \ours in topology structure optimization.  A topology structure is a layout of materials, \eg alloy and concrete, in some designated spatial domain. Given the input from the outside environment, \eg external force, we want to find an optimal structure that achieves the maximum (or minimum)  interested property, \eg stiffness. Topology structure optimization is crucial to many engineering design and manufacturing problems, including 3D printing, and design of air foils, slab bridges, aerodynamic shapes of race cars, \etc The conventional approach is to solve a constraint optimization problem that minimizes a compliance objective subject to a total volume constraint~\citep{sigmund1997design}. However, the numerical computation is usually very costly. We aim to use active learning to learn a model that directly predicts the optimal structure, without the need for running numerical optimization every time. 

We considered the stress experiment in~\citep{keshavarzzadeh2018parametric} with an L-shape linear elastic structure.  The structure is subjected to a load (\ie input) on the bottom right half and is discretized in a $[0, 1] \times [0, 1]$ domain. The load is represented by two parameters, the location (in $[0.5, 1]$) and angle (in $[0, \frac{\pi}{2}]$). The goal is to find the structure that achieves the maximum stiffness given the load. Optimizing the structure  needs to repeatedly call a numerical solver, where the choice of the mesh determines the fidelity.  We used two fidelities to query the training examples. One uses a $50 \times 50$ mesh, the other $75 \times 75$. Correspondingly, the output dimensions are $2,500$ and $5,625$. The costs are measured by the average running time: $\lambda_1 = 1, \lambda_2 = 3$. We randomly generated $500$ structures for test, where the internal solver uses a $100 \times 100$ mesh.  
\begin{figure}[H]
	\centering
	%\setlength\tabcolsep{0.01pt}
	\includegraphics[width=0.48\textwidth]{./figs/rmse_Lbracket.pdf}
	%\vspace{-0.25in}
	\caption{\small Prediction accuracy of active learning in topology structure optimization.}
	\label{fig:tpo}
	%\vspace{-0.2in}
\end{figure}
Initially, we randomly queried $10$ examples at the first fidelity and $2$ at the second fidelity. We then ran all the active learning methods to query $100$ examples. We conducted the experiments for five times, and report the average nRMSE  along with the cost in  Fig. \ref{fig:tpo}. As we can see, \ours achieves much better prediction accuracy than the competing approaches (with the same cost). That implies our predicted structures are much closer to the optimal structures.  While the performance of the other methods tended to converge early, \ours 's performance kept improving and the trend did not stop even when all the queries were finished. It is worth noting that \texttt{MF-BALD} is even worse than random query strategies.  This might because the acquisition function \eqref{eq:mf-bald} does not take  into account the relationships between the fidelities, which are critical for this task. 
  \setlength{\columnsep}{10pt}
  \begin{wrapfigure}{r}{0.5\textwidth}
  	\centering
  	\begin{subfigure}[b]{0.5\textwidth}
  		\centering
  		\includegraphics[width=1.0\linewidth]{figs/topt_ground_v1.eps}
  		\caption{\small Ground Truth}
  		\label{fig:tpo-gt}
  	\end{subfigure}
  	\begin{subfigure}[b]{0.5\textwidth}
  		\centering
  		\includegraphics[width=1.0\linewidth]{figs/topt_mutual_v1.eps}
  		\caption{\small \ours}
  		\label{fig:tpo-ours}
  	\end{subfigure}
  	\begin{subfigure}[b]{0.5\textwidth}
  		\centering
  		\includegraphics[width=1.0\linewidth]{figs/topt_dropout_v1.eps}
  		\caption{\small Dropout-latent}
  		\label{fig:tpo-dropout}
  	\end{subfigure}
  	\begin{subfigure}[b]{0.5\textwidth}
  		\centering
  		\includegraphics[width=1.0\linewidth]{figs/topt_bald_v1.eps}
  		\caption{\small MF-BALD}
  		\label{fig:tpo-bald}
  	\end{subfigure}
  	\begin{subfigure}[b]{0.5\textwidth}
  		\centering
  		\includegraphics[width=1.0\linewidth]{figs/topt_full_random_v1.eps}
  		\caption{\small MF-Random}
  		\label{fig:tpo-random}
  	\end{subfigure}
  	\begin{subfigure}[b]{0.5\textwidth}
  		\centering
  		\includegraphics[width=1.0\linewidth]{figs/topt_fix_random_f1_v1.eps}
  		\caption{\small Random-F1}
  		\label{fig:tpo-random-1}
  	\end{subfigure}
  	\begin{subfigure}[b]{0.5\textwidth}
  		\centering
  		\includegraphics[width=1.0\linewidth]{figs/topt_fix_random_f2_v1.eps}
  		\caption{\small Random-F2}
  		\label{fig:tpo-random-2}
  	\end{subfigure}
  	%	\vspace{-0.3in}
  	\caption{\small The predicted topology structures for $8$ loads. All the active learning approaches started with the same training set (10 fidelity-1 and 2 fidelity-2 examples), and ran with $100$ queries.}
  	\label{fig:pred-top-structure}
  	%\vspace{-0.2in}
  \end{wrapfigure}
To perform a fine-grained comparison, we visualize eight structures predicted by all the methods, after the active learning is finished. As shown in Fig. \ref{fig:pred-top-structure}, \ours predicted much more accurate structures, which capture both the global shapes and local details, and the density of the materials is closer to the ground-truth.  Although \texttt{Dropout-latent} captures the global shapes as well, its predictions are more blurred and miss many local details, \eg the second to seventh structure in Fig. \ref{fig:pred-top-structure}c. The other methods often provided wrong structures (\eg the first and last structure in Fig. \ref{fig:pred-top-structure}d, e, and f) and insufficient density (\eg the second, third and sixth structure in \ref{fig:pred-top-structure}f).

\cmt{  
\begin{figure}[!htb]
	\centering
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_ground_v1.eps}
		\caption{\small Ground Truth}
		\label{fig:tpo-gt}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_mutual_v1.eps}
		\caption{\small \ours}
		\label{fig:tpo-ours}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_dropout_v1.eps}
		\caption{\small Dropout-latent}
		\label{fig:tpo-dropout}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_bald_v1.eps}
		\caption{\small MF-BALD}
		\label{fig:tpo-bald}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_full_random_v1.eps}
		\caption{\small MF-Random}
		\label{fig:tpo-random}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_fix_random_f1_v1.eps}
		\caption{\small Random-F1}
		\label{fig:tpo-random-1}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figs/topt_fix_random_f2_v1.eps}
		\caption{\small Random-F2}
		\label{fig:tpo-random-2}
	\end{subfigure}
%	\vspace{-0.3in}
	\caption{\small The predicted topology structures for $8$ loads. All the active learning approaches started with the same training set (10 fidelity-1 and 2 fidelity-2 examples), and ran with $100$ queries.}
	\label{fig:pred-top-structure}
	%\vspace{-0.2in}
\end{figure}
}
\cmt{
\begin{figure*}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{ccc}
		\setcounter{subfigure}{0}
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/ns_t_1.eps}
			\caption{$t=1$}
		\end{subfigure} &
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/ns_t_5.eps}
			\caption{$t=5$}
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.33\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/ns_t_9.eps}
			\caption{$t=9$}
		\end{subfigure}
	\end{tabular}
	\vspace{-0.05in}
	\caption{\small Examples of the first component of the velocity field (with contour lines) at three time points.} \label{fig:cfd-example}
	\vspace{-0.2in}
\end{figure*}
}
%\vspace{-0.05in}
\subsection{Predicting Fluid Dynamics}
%\vspace{-0.05in}
Third, we applied \ours in a computational fluid dynamics (CFD) problem.  The task is to predict the first component of the velocity field of a flow within a rectangular domain in $[0, 1] \times [0, 1]$. The flow is driven by the boundaries with a prescribed velocity (\ie input)~\citep{bozeman1973numerical}.
Along with time, the local velocities inside the fluid will vary differently, and eventually result in turbulent flows. Computing these fields along with time requires us to solve the incompressive Navier-Stokes equations~\citep{chorin1968numerical}, which is known to be challenging to solve because of their complex behaviors under big Reynolds numbers. We considered active learning with two-fidelity queries to predict the first component of the velocity field  at evenly spaced $20$ time points in $[0, 10]$ (temporal domain). The examples in the first fidelity were generated with a $50 \times 50$ mesh in the spatial domain (\ie $[0, 1]\times [0, 1]$), and the second fidelity $75 \times 75$. The corresponding output dimensions are $50,000$ and $112,500$. The input is a five dimensional vector that consists of the prescribed boundary velocity and Reynold number. See more details in the supplementary material. To collect the test dataset, we randomly sampled $256$ inputs and computed the solution with a $128 \times 128$ mesh. The test outputs are obtained by the cubic-spline interpolation. At the beginning, we randomly queried $10$ and $2$ training examples in the first and second fidelity, respectively. Then we ran each active learning method with $100$ queries. We repeated the experiments for five times. The average nRMSE along with the accumulated cost is shown in Fig. \ref{fig:ns}. It can be seen that during the training, \ours consistently outperforms all the competing methods by a large margin. On the other hand, to achieve the same level of accuracy, \ours spends a much smaller cost. That means, our methods requires much less (high-fidelity) simulations to generate the training examples. This is particularly useful for large-scale CFD applications, in which the simulation is known to be very expensive. 

\begin{figure}[H]
	%\vspace{-0.1in}
	\centering
	%\setlength\tabcolsep{0.01pt}
	\includegraphics[width=0.48\textwidth]{./figs/rmse_Navier.pdf}
	%\vspace{-0.35in}
	\caption{\small Performance of active learning in predicting velocity fields at $20$ time steps in a flow driven by rectangular boundaries. }
	\label{fig:ns}
	%\vspace{-0.18in}
\end{figure}

\zsdc{Finally, we also examined our deep multi-fidelity model in non-active learning. We compared with several state-of-the-art high-dimensional regression models. They all lack effective active learning approaches. Our model consistently outperforms these methods, often by a large margin. This confirms the advantage of our model in surrogate modeling. See the details in the supplementary material.}

==> method.tex <==

\section{Background}

%problem definitions 
\textbf{Problem setting.}  We assume that we can query training examples with $M$ fidelities, which correspond to $M$ mappings, $\{\f_m(\x) \in \mathds{R}^{d_m}\}_{1 \le m \le M}$ where $\x \in \Xcal$ is an $r$-dimensional input, $r$ is small, $d_m$ is the output dimension, often very large, and $\{d_m\}$ are not necessarily identical.  In general, we assume $d_1 \le \ldots \le d_M$.  For instance, in structure design, the input can be  the design parameters. The high fidelity examples correspond to high-resolution structures while the low fidelity ones low-resolution structures.  We denote  by $\lambda_m$ the cost to query with fidelity $m$.  To perform active learning, we begin with a small set of training examples with mixed fidelities. Each step, we select both the fidelity and input location to query new training examples, so as to best balance the learning improvement and computational cost, namely, maximizing the benefit-cost ratio. 
%Assume we can query training examples at different fidelites. Th 
%Note that this is different from popular active learning settings that assume a pool of unlabeled input examples, \eg images. Each time, we only need to rank the inputs and select the top examples to query. 
%Traditional active learning assumes a pool of unlabeled input examples, \eg images. Each time,  these examples will be ranked according to some acquisition (or utility) function computed based on the current model.  We expect the top examples will mostly improve the learning performance. We query the labels of these examples, and add them into the training set to update our model.  

\textbf{Dropout active learning.} A very successful application of active learning with deep neural networks is image classification~\citep{gal2017deep,kirsch2019batchbald}. Typically, a pool of unlabeled input examples, \ie images,  is pre-collected. Each time, we rank the input examples according to an acquisition function computed based on the current model. We then query the labels of the top examples, and add them into the training set. There are two popular acquisition functions. The first one is the predictive entropy of the label, 
\begin{align}
	\mathbb{H}[y|\x, \Dcal] = -\sum_{c} p(y=c|\x, \Dcal) \log p(y=c|\x, \Dcal), \label{eq:image-ac-1}
\end{align}
where $\x$ is the input, and $\Dcal$ are the training data. The other one is BALD (Bayesian active learning by disagreement)~\citep{houlsby2011bayesian} --- the mutual information between the label and model parameters, 
\begin{align}
	\mathbb{I}[y, \btheta|\x, \Dcal]  = \mathbb{H}[y|\x, \Dcal]- \EE_{p(\btheta|\Dcal)}\left[\mathbb{H}(\y|\x, \btheta, \Dcal)\right], \label{eq:image-ac-2}
\end{align}
where $\btheta$ are the NN weights. The computation of these acquisition functions require us to first estimate the posterior of the NN output and weights. A popular approach is to use Monte-Carlo (MC) Dropout~\citep{gal2016dropout}, which can be viewed as a variational inference method of Bayesian NNs. MC Dropout uses a probability $p_i$ to randomly drop the neurons in each layer $i$ (equivalent to zeroing out the corresponding weights) in the forward pass and performs backward pass over the remaining neurons. After training, the weights and output obtained from one such forward pass can be viewed as a sample of the approximate posterior. We can run Dropout multiple times to collect a set of posterior samples and calculate the acquisition functions by Monte-Carlo approximation. 

\vspace{-0.05in}
\section{Deep Multi-Fidelity Modeling for High-Dimensional Outputs}
\vspace{-0.05in}
%summarize the problem, and then proceed.
%Despite the success of Dropout active learning, it can be too expensive for high-dimensional outputs. 
%When the output is a high-dimensional (continuous) vector, it is natural to assume a multivariate Gaussian posterior. The entropy  in XX and XX requires the log determinant of the covariance matrix. However, 
Despite its success, dropout active learning might be inappropriate for high-dimensional (continuous) outputs. When the output is a continuous vector, it is natural to use a multivariate Gaussian posterior, $p(\y|\x, \Dcal) \approx \N(\y|\bmu(\x), \bSigma(\x))$, and the entropy $\mathbb{H}(\y|\x, \Dcal)$ in the acquisition functions  (see \eqref{eq:image-ac-1} and \eqref{eq:image-ac-2}) require us to compute the log determinant of the covariance matrix, $\log|\bSigma(\x)|$. While we can use dropout samples to construct an empirical  estimate $\widehat{\bSigma}(\x)$, due to the large output dimension $n$, the computation of this $n\times n$ matrix and its log determinant is very expensive  or even infeasible. 
One might seek to only estimate the variance of each individual output. However, this will ignore the strong, complex output correlations, which is critical to effectively evaluate the uncertainty and calculate the acquisition function. Furthermore, in our active learning task, we want to optimize the acquisition function to find the best input (rather than rank the inputs in a pre-collected pool). The empirical covariance estimation from random samples can lead to numerical instability in optimization and inconsistent results from different runs. 

To overcome these problems for multi-fidelity active learning, we propose a highly expressive deep multi-fidelity model, for which we develop a structural variational inference method to capture the posterior dependency of the outputs. We propose a novel acquisition function to allow multi-fidelity queries, and develop an efficient, tractable, and reliable approach to calculate the acquisition function. 


Specifically, we use deep neural networks to build a multi-fidelity high-dimensional output model (see Fig. \ref{fig:graphical}) that can flexibly, efficiently capture various complex relationships between the outputs and between the fidelities, taking advantage of these relationships to enhance the predictive performance at the highest fidelity (where we make final predictions).  For each fidelity $m$, we introduce a neural network (NN) that first generates a  $k_m$ dimensional  latent output, and then projects it to the $d_m$ dimensional observed vector, where $k_m \ll d_m$. The NN is parameterized by $\{\W_m, \btheta_m, \A_m\}$ where $\W_m$ is a $k_m \times l_m$ weight matrix in the latent output layer, $\A_m$ is a $d_m \times k_m$ projection matrix, and $\btheta_m$ the weights in all the other layers. Denote by $\x_m$ the NN input, by $\f_m(\x)$ the latent NN output, and by $\y_m(\x)$ the observation. The model is defined by
\begin{align}
	\x_m &= 			[\x; \f_{m-1}(\x)],  \notag \\
	%\x_m &= \begin{matrix*}[l] \x, \;\;(m=1)\\ [\x; \f_{m-1}(\x)],\;\;m>1 \end{matrix*} \notag \\
	%\x_m & = \begin{cases}
	%		\x & m=1,\\
	%		[\x; \f_{m-1}(\x)] & m>1,
	%	\end{cases} \notag \\
	\f_m(\x) &= \W_m\bphi_{\btheta_m}(\x_m),\notag \\
	\y_m(\x) &= \A_m \f_m(\x) + \bepsilon_m, \label{eq:our-model}
\end{align}
where $\bphi_{\btheta_m}$ is the $l_m$ dimensional input to the latent output layer (therefore parameterized by $\btheta_m$), and $\bepsilon_m \sim \N(\bepsilon_m|\0, \sigma^2_m\I)$ is an isotropic Gaussian noise. We set $k_0 = 0$ and so $\f_0(\x)$ is empty; when $m=1$, we have $\x_m = \x$. Note that $\bphi_{\btheta_m}$ can be viewed as a set of nonlinear basis functions. Through their combinations via $\W_m$ and $\A_m$, we can flexibly capture  the complex, strong relationships between the elements of $\y_m$ to improve the prediction. Furthermore,  the input $\x_{m}$ is constructed by appending to the original input $\x$  the latent output $\f_{m-1}$, which can be viewed as a compact  (or low-rank) summary of all the information up to fidelity $m-1$.  After a series of linear and nonlinear transformations, we obtain the latent output $\f_m$ --- the summary up to fidelity $m$ --- and then generate the high dimensional observation $\y_m$. In this way, we efficiently integrate the information from lower fidelities and capture the complex relationship between the current and previous fidelities by learning a nonlinear mapping, $\f_m(\x) = h(\x, \f_{m-1}(\x))$, where $h(\cdot)$ is fulfilled by an NN. %When $m=1$, we set $\x_m = \x$. %The graphical illustration of our model is in Fig. \ref{fig:graphical}.
\begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{./graphic}
	\caption{\small Graphical representation of the deep multi-fidelity model. The low dimensional latent output in each fidelity $\f_m(\x)$ ($1\le m \le M$) is generated by a (deep) neural network.} \label{fig:graphical}
	\vspace{-0.15in}
\end{figure}

%Through a series of linear and nonlinear transformations inside
%the NN, we obtain the output fm(x). In this way, we digest the information from the lower fidelities,
%and capture the complex relationships between the current and previous fidelities by learning a
%nonlinear mapping fm (x) = h(x, fm−1 (x)), where h(·) is fulfilled by the NN. When m = 1, we set
%xm = x. A graphical representation of our model is given in Fig. 1 of the supplementary material.

We place a standard Gaussian prior over the elements in each $\W_m$. Similar to~\citep{snoek2015scalable}, we consider all the remaining parameters as hyper-parameters to ease the posterior inference and uncertainty reasoning. Given the training dataset $\Dcal = \{\{(\x_{nm}, \y_{nm})|m\}_{n=1}^{N_m}\}_m$, the joint probability  of our model is given by
\begin{align}
	&p(\Wcal, \Ycal|\Xcal, \Theta, \s) = \prod\nolimits_{m=1}^M \N\left(\vec(\W_m)|\0, \I\right)\notag \\
	&\cdot \prod\nolimits_{n=1}^{N_m} \N\big(\y_{nm}|\A_m \f_m(\x_{nm}), \sigma_m^2\I\big), \label{eq:joint-prob}
\end{align}
where $\Wcal = \{\W_m\}_{1\le m\le M}$,  $\Theta=\{\btheta_m, \A_m\}_{1\le m \le M}$, $\s = [\sigma^2_1, \ldots, \sigma^2_M]^\top$, and $\{\Xcal$, $\Ycal\}$ are the inputs and outputs in $\Dcal$. 

To estimate the posterior of our model (which is used to calculate the acquisition function and query new examples), we develop a stochastic structural variational learning algorithm. Specifically, for each $\W_m$,  we introduce a multivariate Gaussian posterior, $q(\W_m) = \N\left(\vec(\W_m)|\bmu_m, \bSigma_m\right)$.  To ensure the positive definiteness, we parameterize  $\bSigma_m$ by its Cholesky decomposition, $\bSigma_m = \L_m \L_m^\top$, where $\L_m$ is a lower triangular matrix. We then assume the posterior $q(\Wcal) =\prod_{m=1}^M q(\W_m)$, and construct a variational model evidence lower bound (ELBO)~\citep{wainwright2008graphical}, %$\Lcal\big(q(\Wcal), \Theta, \s\big) = \EE_{q}[ \log(p(\Wcal, \Ycal|\Xcal, \Theta, \s)/q(\Wcal))]$. 
\begin{align}
	&\Lcal\big(q(\Wcal), \Theta, \s\big) = \EE_{q}\left[ \log\frac{p(\Wcal, \Ycal|\Xcal, \Theta, \s)}{q(\Wcal)}\right] \notag \\
	&=-\text{KL}\big(q(\Wcal)\|p(\Wcal)\big) \notag \\
	&+ \sum_{m=1}^M\sum_{n=1}^{N_m} \EE_q\left[\log \N(\y_{nm}|\A_m \f_m(\x_{nm}),\sigma_m^2\I)\right], \label{eq:elbo}
\end{align}
where $\text{KL}(\cdot \| \cdot)$ is Kullback Leibler divergence and $p(\Wcal)$ the prior of $\Wcal$. We maximize $\Lcal$ to jointly estimate $q(\Wcal)$ and the hyper-parameters. While $\Lcal$ is intractable, it is straightforward to use the reparameterization trick~\citep{kingma2013auto} to generate parameterized samples for each $\vec(\W_m)$: $\bmu_m + \L_m \bxi_m$ where $\bxi_m \sim \N(\0, \I)$, substitute them into \eqref{eq:elbo} to obtain a stochastic estimate of $\Lcal$,  and perform efficient stochastic optimization. %We left the details in the supplementary material. 

%multi-fidelit queries
\vspace{-0.1in}
\section{Multi-Fidelity Active Learning}
\vspace{-0.1in}
\subsection{Mutual Information based Acquisition Function}
\vspace{-0.1in}
We now consider how to perform active learning with multi-fidelity queries. We assume that at each fidelity $m$, the most valuable training example is the one that can best improve our final prediction, namely, the prediction at the highest fidelity $M$. 
To this end, we propose our acquisition function based on the mutual information between the outputs at fidelity $m$ and $M$,
\begin{align}
	&a(\x, m)  = \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right) \label{eq:ac} \\
	&= \frac{1}{\lambda_m} \big(\mathbb{H}(\y_m|\Dcal) +\mathbb{H}(\y_M|\Dcal) - \mathbb{H}(\y_m, \y_M|\Dcal) \big), \notag
\end{align}
%\begin{align}
%	a(\x, m)  &= \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right), \notag \\
%	&= \frac{1}{\lambda_m} \left(\mathbb{H}(\y_m(\x)|\Dcal) +\mathbb{H}(\y_M(\x)|\Dcal) - \mathbb{H}(\y_m(\x), \y_M(\x)|\Dcal) \right) \label{eq:ac}
%\end{align}
where $\lambda_m>0$ is the cost of querying a training example with fidelity $m$. When $m=M$, we have $a(\x, M) = \frac{1}{\lambda_M} \mathbb{H}\left(\y_M(\x)|\Dcal\right)$ ---  the output entropy.  Therefore, our acquisition function is an extension of the popular predictive entropy principle in conventional active learning.  At each step, we maximize our acquisition function to identify a pair of fidelity and input location that give the biggest benefit-cost ratio.  %Note that we can also adjust the BALD principle [??] in the multi-fidelity setting,  $a_{\text{BALD}} = \frac{1}{\lambda_m}$ However, given all the parameters, the uncertainty of the output only comes form the Gaussian noise, ....

%talk about BALD

%challengen, our method
\vspace{-0.1in}
\subsection{Efficient Acquisition Function Calculation}\label{sect:ac-compute}
\vspace{-0.1in}
To maximize the acquisition function \eqref{eq:ac}, a critical challenge is to compute the posterior of the outputs $\{\y_m\}$ in every fidelity, based on our model estimation results, $p(\Wcal|\Dcal) \approx q(\Wcal)$.  Due to high dimensionality of each $\y_m$ and the nonlinear coupling of the latent outputs across the fidelities (see \eqref{eq:our-model}), the computation is challenging and analytically intractable.  To address this issue, we first consider approximating the posterior of the low dimensional latent output $\f_m$, which can be viewed a function of the random NN weights $\bOmega_m = \{\W_1, \ldots, \W_m\}$ (given the input $\x$). We use multivariate Delta's method~\citep{oehlert1992note,bickel2015mathematical} to compute the moments of $\f_m$. Specifically, we approximate $\f_m$ with a first-order Taylor expansion, 
\begin{align}
	\f_m(\bOmega_m) \approx \f_m(\EE[\bOmega_m]) + \J_m\left(\boldeta_m  - \EE[\boldeta_m]\right), \label{eq:1order}
\end{align}
where the expectation is under $q(\cdot)$,  $\boldeta_m = \vec(\bOmega_m)$, $\J_m = \frac{\partial \f_m}{\partial \boldeta_m}|_{\boldeta_m = \EE[\boldeta_m]}$ is the Jacobian matrix at the mean.  The rationale is as follows. First, $\f_m$ is linear to $\W_m$, and the second-order derivative is simply $\0$.  Second, as the NN output, $\f_m$ is highly nonlinear to the random weights in previous layers, \ie $\W_j$ ($j<m$). Hence, we can assume the change rate of $\f_m$ (\eg gradient or Jacobian) has much greater scales than the posterior covariance of $\W_j$ in the second-order term of the Taylor expansion. Note that $q(\W_j)$ is much more informative and hence much more concentrated than the prior $ \N(\vec(\W_j)|\0, \I)$. The scale of the posterior covariance should be much less than $1$. Integrating both cases, the first-order term can dominate the Taylor expansion and hence we ignore the higher order terms. 
Based on \eqref{eq:1order}, we can easily calculate the first and second moments of $\f_m$, 
\begin{align}
	\balpha_m &= \EE[\f_m] \approx \f_m\left(\EE[\bOmega_m]\right), \notag \\
	\V_m &= \text{cov}[\f_m] \approx \J_m \text{cov}(\boldeta_m) \J_m^\top, 
\end{align}
where  $\text{cov}(\boldeta_m) = \diag\left(\left\{\text{cov}\big(\vec(\W_j)\big)\right\}_{1\le j\le m}\right)$. 
Then we use moment matching to estimate a joint Gaussian posterior, $q(\f_m)  = \N(\f_m|\balpha_m, \V_m)$. Next, according to our model definition \eqref{eq:our-model}, we can obtain the posterior of the ouptut $\y_m$, 
\begin{align}
	q(\y_m) = \N(\y_m|\A_m \balpha_m, \A_m \V_m \A_m^\top + \sigma_m^2\I).
\end{align}
The output entropy is  $\mathbb{H}(\y_m|\Dcal) = \frac{1}{2}\log|\A_m \V_m \A_m^\top + \sigma_m^2\I| + d_m \log\sqrt{2\pi e}$.  However, directly computing the log determinant of a $d_m \times d_m$ matrix is very expensive. We further use the Weinstein-Aronszajn identity~\citep{kato2013perturbation} to derive 
\begin{align}
	&\mathbb{H}(\y_m|\Dcal) =  \frac{1}{2}\log|\sigma_m^{-2}\A_m \V_m \A_m^\top + \I|  + d_m \log \sqrt{2\pi e\sigma_m^2} \notag \\
	&=\frac{1}{2}\log|\sigma_m^{-2}\A_m^\top\A_m\V_m + \I| + d_m \log \sqrt{2\pi e\sigma_m^2}. \label{eq:en_ym}
\end{align}
Now, the log determinant is calculated on a much smaller, $k_m \times k_m$ matrix, which is very cheap and efficient. 

Using a similar approach, we can calculate the joint posterior of $\barf_m = [\f_m; \f_M]$ and then $\bary_m=[\y_m; \y_M]$.  First, we view $\barf_m$ as a function of all the random weights, $\Wcal = \{\W_1, \ldots, \W_M\}$. We use the multivariate Delta's method and moment matching to estimate a joint Gaussian posterior, 
$q(\barf_m) = \N(\barf_m|\baralpha_m, \barV_m)$ where $\baralpha_m = \barf_m\left(\EE[\Wcal]\right)$,  $\barV_m = \barJ_m \text{cov}(\boldeta)\barJ_m^\top$, $\boldeta = \vec(\Wcal)$, $\barJ_m = \frac{\partial \barf_m}{\partial \boldeta}|_{\boldeta = \EE[\boldeta]}$, and $\text{cov}(\boldeta) = \diag\left(\left\{\text{cov}\big(\vec(\W_j)\big)\right\}_{1\le j\le M}\right)$. According to our model, we can represent
\[
\bary_m = \barA_m \barf_m + \bareps_m,
\]
where $\barA_m = \diag(\A_m, \A_M)$ and $\bareps_m = [\bepsilon_m; \bepsilon_M]$. Therefore, the joint posterior of $\bary_m$ is 
\begin{align}
	q(\bary_m) = \N(\bary_m|\barA_m \baralpha_m, \barA_m \barV_m \barA_m^\top + \S_m),
\end{align}
where $\S_m = \diag(\sigma^2_m\I_{d_m}, \sigma^2_M \I_{d_M})$,  $\I_{d_m}$ and $\I_{d_M}$ are identity matrices of $d_m \times d_m$ and $d_M \times d_M$, respectively.  Again, we use  Weinstein-Aronszajn identity to simplify the entropy computation of $\bary_m$ (\ie $\y_m$ and $\y_M$), 
\begin{align}
	&\mathbb{H}(\y_m, \y_M|\Dcal)  =\frac{1}{2}\log|\S_m^{-1}\barA_m \barV_m \barA_m^\top + \I|  + \xi_m \notag \\
	&=\frac{1}{2}\log|\barA_m^\top \S_m^{-1} \barA_m \barV_m + \I| + \xi_m, \label{eq:en_ymM}
\end{align}
where $\xi_m = d_m \log \sqrt{2\pi e\sigma_m^2} + d_M \log \sqrt{2\pi e\sigma_M^2}$ and the log determinant is computed from a $(k_m + k_M) \times (k_m + k_M)$ matrix, which is cheap and efficient. Note that we can use matrix blocks to compute $\barA_m^\top \S_m^{-1} \barA_m = \diag\left(\sigma_m^{-2}\A_m^\top \A_m, \sigma_M^{-2}\A_M^\top \A_M\right)$.

Now, based on \eqref{eq:en_ym} and \eqref{eq:en_ymM}, we can calculate our acquisition function \eqref{eq:ac} in an analytic and deterministic way. For each fidelity $m$, we maximize $a(\x, m)$ w.r.t to $\x$ to find the optimal input. We can use automatic differential libraries to calculate the gradient and feed it to any optimization algorithm, \eg L-BFGS.   We then use the optimal input at the fidelity that has the largest acquisition function value to query  the next training example. Our deep multi-fidelity active learning is summarized in Algorithm \ref{alg:dmf-al}. 
%problem of dropout ... 
\setlength{\textfloatsep}{0.05cm}
\begin{algorithm}                      % enter the algorithm environment
	\small
	\caption{\ours($\Dcal$, $T$, $\{\lambda_m\}_{m=1}^M$ )}          
	\label{alg:dmf-al}                           
	\begin{algorithmic}[1]                    % enter the algorithmic environment
		\STATE Train the deep multi-fidelity model \eqref{eq:joint-prob} on the initial dataset $\Dcal$ with stochastic structural variational learning.  
		\FOR {$t=1,\ldots, T$}
		\STATE Based on \eqref{eq:en_ym} and \eqref{eq:en_ymM}, calculate and optimize the acquisition function \eqref{eq:ac} to find 
		\begin{align}
			(\x_{t}, m_{t}) = \argmax_{\x \in \Xcal, 1\le m \le M} a(\x, m).\notag % =  \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right).\notag
		\end{align}
		\STATE Query the output $\y_{t}$ with fidelity $m_t$.
		\STATE $\Dcal \leftarrow \Dcal \cup \{(\x_{t}, \y_{t})|m_t\}$.
		\STATE Re-train the deep multi-fidelity model on $\Dcal$.
		\ENDFOR
		%\vspace{-0.05in}
		%\RETURN the current posterior $q_{cur}(\cdot)$.
	\end{algorithmic}
\end{algorithm}
\setlength{\floatsep}{0.1cm}
\vspace{-0.05in}
\subsection{Algorithm Complexity}
\vspace{-0.05in}
The time complexity of training our deep multi-fidelity model is $\Ocal(N(\sum_{m=1}^M (k_ml_m)^2 + F))$ where $N$ and $F$ are the total number of training examples and NN parameters, respectively. The space complexity is $\Ocal(F + \sum_{m=1}^M (k_ml_m)^2)$, which is to store the NN parameters, and posterior mean and covariance of each random weight matrix $\W_m$. The time complexity of calculating the acquisition function is $\Ocal(\sum_{m=1}^M d_mk_m^2 + k_m^3)$. Since $k_m \ll d_m$, the complexity is linear to the output dimensions. Due to the usage of the learned variational posterior $q(\Wcal)$, the space complexity of computing the acquisition function is the same as that of training the multi-fidelity model.


==> method_copy.tex <==

\section{Background}

%problem definitions 
\textbf{Problem setting.}  We assume that we can query training examples with $M$ fidelities, which correspond to $M$ mappings, $\{\f_m(\x) \in \mathds{R}^{d_m}\}_{1 \le m \le M}$ where $\x \in \Xcal$ is an $r$-dimensional input, $r$ is small, $d_m$ is the output dimension, often very large, and $\{d_m\}$ are not necessarily identical.  In general, we assume $d_1 \le \ldots \le d_M$.  For instance, in structure design, the input can be  the design parameters. The high fidelity examples correspond to high-resolution structures while the low fidelity ones low-resolution structures.  We denote  by $\lambda_m$ the cost to query with fidelity $m$.  To perform active learning, we begin with a small set of training examples with mixed fidelities. Each step, we select both the fidelity and input location to query new training examples, so as to best balance the learning improvement and computational cost, namely, maximizing the benefit-cost ratio. 
%Assume we can query training examples at different fidelites. Th 
%Note that this is different from popular active learning settings that assume a pool of unlabeled input examples, \eg images. Each time, we only need to rank the inputs and select the top examples to query. 
%Traditional active learning assumes a pool of unlabeled input examples, \eg images. Each time,  these examples will be ranked according to some acquisition (or utility) function computed based on the current model.  We expect the top examples will mostly improve the learning performance. We query the labels of these examples, and add them into the training set to update our model.  

\textbf{Dropout active learning.} A very successful application of active learning with deep neural networks is image classification~\citep{gal2017deep,kirsch2019batchbald}. Typically, a pool of unlabeled input examples, \ie images,  is pre-collected. Each time, we rank the input examples according to an acquisition function computed based on the current model. We then query the labels of the top examples, and add them into the training set. There are two popular acquisition functions. The first one is the predictive entropy of the label, 
\begin{align}
	\mathbb{H}[y|\x, \Dcal] = -\sum_{c} p(y=c|\x, \Dcal) \log p(y=c|\x, \Dcal), \label{eq:image-ac-1}
\end{align}
where $\x$ is the input, and $\Dcal$ are the training data. The other one is BALD (Bayesian active learning by disagreement)~\citep{houlsby2011bayesian} --- the mutual information between the label and model parameters, 
\begin{align}
	\mathbb{I}[y, \btheta|\x, \Dcal]  = \mathbb{H}[y|\x, \Dcal]- \EE_{p(\btheta|\Dcal)}\left[\mathbb{H}(\y|\x, \btheta, \Dcal)\right], \label{eq:image-ac-2}
\end{align}
where $\btheta$ are the NN weights. The computation of these acquisition functions require us to first estimate the posterior of the NN output and weights. A popular approach is to use Monte-Carlo (MC) Dropout~\citep{gal2016dropout}, which can be viewed as a variational inference method of Bayesian NNs. MC Dropout uses a probability $p_i$ to randomly drop the neurons in each layer $i$ (equivalent to zeroing out the corresponding weights) in the forward pass and performs backward pass over the remaining neurons. After training, the weights and output obtained from one such forward pass can be viewed as a sample of the approximate posterior. We can run Dropout multiple times to collect a set of posterior samples and calculate the acquisition functions by Monte-Carlo approximation. 

\vspace{-0.05in}
\section{Deep Multi-Fidelity Modeling for High-Dimensional Outputs}
\vspace{-0.05in}
%summarize the problem, and then proceed.
%Despite the success of Dropout active learning, it can be too expensive for high-dimensional outputs. 
%When the output is a high-dimensional (continuous) vector, it is natural to assume a multivariate Gaussian posterior. The entropy  in XX and XX requires the log determinant of the covariance matrix. However, 
Despite its success, dropout active learning might be inappropriate for high-dimensional (continuous) outputs. When the output is a continuous vector, it is natural to use a multivariate Gaussian posterior, $p(\y|\x, \Dcal) \approx \N(\y|\bmu(\x), \bSigma(\x))$, and the entropy $\mathbb{H}(\y|\x, \Dcal)$ in the acquisition functions  (see \eqref{eq:image-ac-1} and \eqref{eq:image-ac-2}) require us to compute the log determinant of the covariance matrix, $\log|\bSigma(\x)|$. While we can use dropout samples to construct an empirical  estimate $\widehat{\bSigma}(\x)$, due to the large output dimension $n$, the computation of this $n\times n$ matrix and its log determinant is very expensive  or even infeasible. 
One might seek to only estimate the variance of each individual output. However, this will ignore the strong, complex output correlations, which is critical to effectively evaluate the uncertainty and calculate the acquisition function. Furthermore, in our active learning task, we want to optimize the acquisition function to find the best input (rather than rank the inputs in a pre-collected pool). The empirical covariance estimation from random samples can lead to numerical instability in optimization and inconsistent results from different runs. 

To overcome these problems for multi-fidelity active learning, we propose a highly expressive deep multi-fidelity model, for which we develop a structural variational inference method to capture the posterior dependency of the outputs. We propose a novel acquisition function to allow multi-fidelity queries, and develop an efficient, tractable, and reliable approach to calculate the acquisition function. 


Specifically, we use deep neural networks to build a multi-fidelity high-dimensional output model (see Fig. \ref{fig:graphical}) that can flexibly, efficiently capture various complex relationships between the outputs and between the fidelities, taking advantage of these relationships to enhance the predictive performance at the highest fidelity (where we make final predictions).  For each fidelity $m$, we introduce a neural network (NN) that first generates a  $k_m$ dimensional  latent output, and then projects it to the $d_m$ dimensional observed vector, where $k_m \ll d_m$. The NN is parameterized by $\{\W_m, \btheta_m, \A_m\}$ where $\W_m$ is a $k_m \times l_m$ weight matrix in the latent output layer, $\A_m$ is a $d_m \times k_m$ projection matrix, and $\btheta_m$ the weights in all the other layers. Denote by $\x_m$ the NN input, by $\f_m(\x)$ the latent NN output, and by $\y_m(\x)$ the observation. The model is defined by
\begin{align}
	\x_m &= 			[\x; \f_{m-1}(\x)],  \notag \\
	%\x_m &= \begin{matrix*}[l] \x, \;\;(m=1)\\ [\x; \f_{m-1}(\x)],\;\;m>1 \end{matrix*} \notag \\
	%\x_m & = \begin{cases}
	%		\x & m=1,\\
	%		[\x; \f_{m-1}(\x)] & m>1,
	%	\end{cases} \notag \\
	\f_m(\x) &= \W_m\bphi_{\btheta_m}(\x_m),\notag \\
	\y_m(\x) &= \A_m \f_m(\x) + \bepsilon_m, \label{eq:our-model}
\end{align}
where $\bphi_{\btheta_m}$ is the $l_m$ dimensional input to the latent output layer (therefore parameterized by $\btheta_m$), and $\bepsilon_m \sim \N(\bepsilon_m|\0, \sigma^2_m\I)$ is an isotropic Gaussian noise. We set $k_0 = 0$ and so $\f_0(\x)$ is empty; when $m=1$, we have $\x_m = \x$. Note that $\bphi_{\btheta_m}$ can be viewed as a set of nonlinear basis functions. Through their combinations via $\W_m$ and $\A_m$, we can flexibly capture  the complex, strong relationships between the elements of $\y_m$ to improve the prediction. Furthermore,  the input $\x_{m}$ is constructed by appending to the original input $\x$  the latent output $\f_{m-1}$, which can be viewed as a compact  (or low-rank) summary of all the information up to fidelity $m-1$.  After a series of linear and nonlinear transformations, we obtain the latent output $\f_m$ --- the summary up to fidelity $m$ --- and then generate the high dimensional observation $\y_m$. In this way, we efficiently integrate the information from lower fidelities and capture the complex relationship between the current and previous fidelities by learning a nonlinear mapping, $\f_m(\x) = h(\x, \f_{m-1}(\x))$, where $h(\cdot)$ is fulfilled by an NN. %When $m=1$, we set $\x_m = \x$. %The graphical illustration of our model is in Fig. \ref{fig:graphical}.
\begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{./graphic}
	\caption{\small Graphical representation of the deep multi-fidelity model. The low dimensional latent output in each fidelity $\f_m(\x)$ ($1\le m \le M$) is generated by a (deep) neural network.} \label{fig:graphical}
	\vspace{-0.15in}
\end{figure}

%Through a series of linear and nonlinear transformations inside
%the NN, we obtain the output fm(x). In this way, we digest the information from the lower fidelities,
%and capture the complex relationships between the current and previous fidelities by learning a
%nonlinear mapping fm (x) = h(x, fm−1 (x)), where h(·) is fulfilled by the NN. When m = 1, we set
%xm = x. A graphical representation of our model is given in Fig. 1 of the supplementary material.

We place a standard Gaussian prior over the elements in each $\W_m$. Similar to~\citep{snoek2015scalable}, we consider all the remaining parameters as hyper-parameters to ease the posterior inference and uncertainty reasoning. Given the training dataset $\Dcal = \{\{(\x_{nm}, \y_{nm})|m\}_{n=1}^{N_m}\}_m$, the joint probability  of our model is given by
\begin{align}
	&p(\Wcal, \Ycal|\Xcal, \Theta, \s) = \prod\nolimits_{m=1}^M \N\left(\vec(\W_m)|\0, \I\right)\notag \\
	&\cdot \prod\nolimits_{n=1}^{N_m} \N\big(\y_{nm}|\A_m \f_m(\x_{nm}), \sigma_m^2\I\big), \label{eq:joint-prob}
\end{align}
where $\Wcal = \{\W_m\}_{1\le m\le M}$,  $\Theta=\{\btheta_m, \A_m\}_{1\le m \le M}$, $\s = [\sigma^2_1, \ldots, \sigma^2_M]^\top$, and $\{\Xcal$, $\Ycal\}$ are the inputs and outputs in $\Dcal$. 

To estimate the posterior of our model (which is used to calculate the acquisition function and query new examples), we develop a stochastic structural variational learning algorithm. Specifically, for each $\W_m$,  we introduce a multivariate Gaussian posterior, $q(\W_m) = \N\left(\vec(\W_m)|\bmu_m, \bSigma_m\right)$.  To ensure the positive definiteness, we parameterize  $\bSigma_m$ by its Cholesky decomposition, $\bSigma_m = \L_m \L_m^\top$, where $\L_m$ is a lower triangular matrix. We then assume the posterior $q(\Wcal) =\prod_{m=1}^M q(\W_m)$, and construct a variational model evidence lower bound (ELBO)~\citep{wainwright2008graphical}, %$\Lcal\big(q(\Wcal), \Theta, \s\big) = \EE_{q}[ \log(p(\Wcal, \Ycal|\Xcal, \Theta, \s)/q(\Wcal))]$. 
\begin{align}
	&\Lcal\big(q(\Wcal), \Theta, \s\big) = \EE_{q}\left[ \log\frac{p(\Wcal, \Ycal|\Xcal, \Theta, \s)}{q(\Wcal)}\right] \notag \\
	&=-\text{KL}\big(q(\Wcal)\|p(\Wcal)\big) \notag \\
	&+ \sum_{m=1}^M\sum_{n=1}^{N_m} \EE_q\left[\log \N(\y_{nm}|\A_m \f_m(\x_{nm}),\sigma_m^2\I)\right], \label{eq:elbo}
\end{align}
where $\text{KL}(\cdot \| \cdot)$ is Kullback Leibler divergence and $p(\Wcal)$ the prior of $\Wcal$. We maximize $\Lcal$ to jointly estimate $q(\Wcal)$ and the hyper-parameters. While $\Lcal$ is intractable, it is straightforward to use the reparameterization trick~\citep{kingma2013auto} to generate parameterized samples for each $\vec(\W_m)$: $\bmu_m + \L_m \bxi_m$ where $\bxi_m \sim \N(\0, \I)$, substitute them into \eqref{eq:elbo} to obtain a stochastic estimate of $\Lcal$,  and perform efficient stochastic optimization. %We left the details in the supplementary material. 

%multi-fidelit queries
\vspace{-0.1in}
\section{Multi-Fidelity Active Learning}
\vspace{-0.1in}
\subsection{Mutual Information based Acquisition Function}
\vspace{-0.1in}
We now consider how to perform active learning with multi-fidelity queries. We assume that at each fidelity $m$, the most valuable training example is the one that can best improve our final prediction, namely, the prediction at the highest fidelity $M$. 
To this end, we propose our acquisition function based on the mutual information between the outputs at fidelity $m$ and $M$,
\begin{align}
	&a(\x, m)  = \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right) \label{eq:ac} \\
	&= \frac{1}{\lambda_m} \big(\mathbb{H}(\y_m|\Dcal) +\mathbb{H}(\y_M|\Dcal) - \mathbb{H}(\y_m, \y_M|\Dcal) \big), \notag
\end{align}
%\begin{align}
%	a(\x, m)  &= \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right), \notag \\
%	&= \frac{1}{\lambda_m} \left(\mathbb{H}(\y_m(\x)|\Dcal) +\mathbb{H}(\y_M(\x)|\Dcal) - \mathbb{H}(\y_m(\x), \y_M(\x)|\Dcal) \right) \label{eq:ac}
%\end{align}
where $\lambda_m>0$ is the cost of querying a training example with fidelity $m$. When $m=M$, we have $a(\x, M) = \frac{1}{\lambda_M} \mathbb{H}\left(\y_M(\x)|\Dcal\right)$ ---  the output entropy.  Therefore, our acquisition function is an extension of the popular predictive entropy principle in conventional active learning.  At each step, we maximize our acquisition function to identify a pair of fidelity and input location that give the biggest benefit-cost ratio.  %Note that we can also adjust the BALD principle [??] in the multi-fidelity setting,  $a_{\text{BALD}} = \frac{1}{\lambda_m}$ However, given all the parameters, the uncertainty of the output only comes form the Gaussian noise, ....

%talk about BALD

%challengen, our method
\vspace{-0.1in}
\subsection{Efficient Acquisition Function Calculation}\label{sect:ac-compute}
\vspace{-0.1in}
To maximize the acquisition function \eqref{eq:ac}, a critical challenge is to compute the posterior of the outputs $\{\y_m\}$ in every fidelity, based on our model estimation results, $p(\Wcal|\Dcal) \approx q(\Wcal)$.  Due to high dimensionality of each $\y_m$ and the nonlinear coupling of the latent outputs across the fidelities (see \eqref{eq:our-model}), the computation is challenging and analytically intractable.  To address this issue, we first consider approximating the posterior of the low dimensional latent output $\f_m$, which can be viewed a function of the random NN weights $\bOmega_m = \{\W_1, \ldots, \W_m\}$ (given the input $\x$). We use multivariate Delta's method~\citep{oehlert1992note,bickel2015mathematical} to compute the moments of $\f_m$. Specifically, we approximate $\f_m$ with a first-order Taylor expansion, 
\begin{align}
	\f_m(\bOmega_m) \approx \f_m(\EE[\bOmega_m]) + \J_m\left(\boldeta_m  - \EE[\boldeta_m]\right), \label{eq:1order}
\end{align}
where the expectation is under $q(\cdot)$,  $\boldeta_m = \vec(\bOmega_m)$, $\J_m = \frac{\partial \f_m}{\partial \boldeta_m}|_{\boldeta_m = \EE[\boldeta_m]}$ is the Jacobian matrix at the mean.  The rationale is as follows. First, $\f_m$ is linear to $\W_m$, and the second-order derivative is simply $\0$.  Second, as the NN output, $\f_m$ is highly nonlinear to the random weights in previous layers, \ie $\W_j$ ($j<m$). Hence, we can assume the change rate of $\f_m$ (\eg gradient or Jacobian) has much greater scales than the posterior covariance of $\W_j$ in the second-order term of the Taylor expansion. Note that $q(\W_j)$ is much more informative and hence much more concentrated than the prior $ \N(\vec(\W_j)|\0, \I)$. The scale of the posterior covariance should be much less than $1$. Integrating both cases, the first-order term can dominate the Taylor expansion and hence we ignore the higher order terms. 
Based on \eqref{eq:1order}, we can easily calculate the first and second moments of $\f_m$, 
\begin{align}
	\balpha_m &= \EE[\f_m] \approx \f_m\left(\EE[\bOmega_m]\right), \notag \\
	\V_m &= \text{cov}[\f_m] \approx \J_m \text{cov}(\boldeta_m) \J_m^\top, 
\end{align}
where  $\text{cov}(\boldeta_m) = \diag\left(\left\{\text{cov}\big(\vec(\W_j)\big)\right\}_{1\le j\le m}\right)$. 
Then we use moment matching to estimate a joint Gaussian posterior, $q(\f_m)  = \N(\f_m|\balpha_m, \V_m)$. Next, according to our model definition \eqref{eq:our-model}, we can obtain the posterior of the ouptut $\y_m$, 
\begin{align}
	q(\y_m) = \N(\y_m|\A_m \balpha_m, \A_m \V_m \A_m^\top + \sigma_m^2\I).
\end{align}
The output entropy is  $\mathbb{H}(\y_m|\Dcal) = \frac{1}{2}\log|\A_m \V_m \A_m^\top + \sigma_m^2\I| + d_m \log\sqrt{2\pi e}$.  However, directly computing the log determinant of a $d_m \times d_m$ matrix is very expensive. We further use the Weinstein-Aronszajn identity~\citep{kato2013perturbation} to derive 
\begin{align}
	&\mathbb{H}(\y_m|\Dcal) =  \frac{1}{2}\log|\sigma_m^{-2}\A_m \V_m \A_m^\top + \I|  + d_m \log \sqrt{2\pi e\sigma_m^2} \notag \\
	&=\frac{1}{2}\log|\sigma_m^{-2}\A_m^\top\A_m\V_m + \I| + d_m \log \sqrt{2\pi e\sigma_m^2}. \label{eq:en_ym}
\end{align}
Now, the log determinant is calculated on a much smaller, $k_m \times k_m$ matrix, which is very cheap and efficient. 

Using a similar approach, we can calculate the joint posterior of $\barf_m = [\f_m; \f_M]$ and then $\bary_m=[\y_m; \y_M]$.  First, we view $\barf_m$ as a function of all the random weights, $\Wcal = \{\W_1, \ldots, \W_M\}$. We use the multivariate Delta's method and moment matching to estimate a joint Gaussian posterior, 
$q(\barf_m) = \N(\barf_m|\baralpha_m, \barV_m)$ where $\baralpha_m = \barf_m\left(\EE[\Wcal]\right)$,  $\barV_m = \barJ_m \text{cov}(\boldeta)\barJ_m^\top$, $\boldeta = \vec(\Wcal)$, $\barJ_m = \frac{\partial \barf_m}{\partial \boldeta}|_{\boldeta = \EE[\boldeta]}$, and $\text{cov}(\boldeta) = \diag\left(\left\{\text{cov}\big(\vec(\W_j)\big)\right\}_{1\le j\le M}\right)$. According to our model, we can represent
\[
\bary_m = \barA_m \barf_m + \bareps_m,
\]
where $\barA_m = \diag(\A_m, \A_M)$ and $\bareps_m = [\bepsilon_m; \bepsilon_M]$. Therefore, the joint posterior of $\bary_m$ is 
\begin{align}
	q(\bary_m) = \N(\bary_m|\barA_m \baralpha_m, \barA_m \barV_m \barA_m^\top + \S_m),
\end{align}
where $\S_m = \diag(\sigma^2_m\I_{d_m}, \sigma^2_M \I_{d_M})$,  $\I_{d_m}$ and $\I_{d_M}$ are identity matrices of $d_m \times d_m$ and $d_M \times d_M$, respectively.  Again, we use  Weinstein-Aronszajn identity to simplify the entropy computation of $\bary_m$ (\ie $\y_m$ and $\y_M$), 
\begin{align}
	&\mathbb{H}(\y_m, \y_M|\Dcal)  =\frac{1}{2}\log|\S_m^{-1}\barA_m \barV_m \barA_m^\top + \I|  + \xi_m \notag \\
	&=\frac{1}{2}\log|\barA_m^\top \S_m^{-1} \barA_m \barV_m + \I| + \xi_m, \label{eq:en_ymM}
\end{align}
where $\xi_m = d_m \log \sqrt{2\pi e\sigma_m^2} + d_M \log \sqrt{2\pi e\sigma_M^2}$ and the log determinant is computed from a $(k_m + k_M) \times (k_m + k_M)$ matrix, which is cheap and efficient. Note that we can use matrix blocks to compute $\barA_m^\top \S_m^{-1} \barA_m = \diag\left(\sigma_m^{-2}\A_m^\top \A_m, \sigma_M^{-2}\A_M^\top \A_M\right)$.

Now, based on \eqref{eq:en_ym} and \eqref{eq:en_ymM}, we can calculate our acquisition function \eqref{eq:ac} in an analytic and deterministic way. For each fidelity $m$, we maximize $a(\x, m)$ w.r.t to $\x$ to find the optimal input. We can use automatic differential libraries to calculate the gradient and feed it to any optimization algorithm, \eg L-BFGS.   We then use the optimal input at the fidelity that has the largest acquisition function value to query  the next training example. Our deep multi-fidelity active learning is summarized in Algorithm \ref{alg:dmf-al}. 
%problem of dropout ... 
\setlength{\textfloatsep}{0.05cm}
\begin{algorithm}                      % enter the algorithm environment
	\small
	\caption{\ours($\Dcal$, $T$, $\{\lambda_m\}_{m=1}^M$ )}          
	\label{alg:dmf-al}                           
	\begin{algorithmic}[1]                    % enter the algorithmic environment
		\STATE Train the deep multi-fidelity model \eqref{eq:joint-prob} on the initial dataset $\Dcal$ with stochastic structural variational learning.  
		\FOR {$t=1,\ldots, T$}
		\STATE Based on \eqref{eq:en_ym} and \eqref{eq:en_ymM}, calculate and optimize the acquisition function \eqref{eq:ac} to find 
		\begin{align}
			(\x_{t}, m_{t}) = \argmax_{\x \in \Xcal, 1\le m \le M} a(\x, m).\notag % =  \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right).\notag
		\end{align}
		\STATE Query the output $\y_{t}$ with fidelity $m_t$.
		\STATE $\Dcal \leftarrow \Dcal \cup \{(\x_{t}, \y_{t})|m_t\}$.
		\STATE Re-train the deep multi-fidelity model on $\Dcal$.
		\ENDFOR
		%\vspace{-0.05in}
		%\RETURN the current posterior $q_{cur}(\cdot)$.
	\end{algorithmic}
\end{algorithm}
\setlength{\floatsep}{0.1cm}
\vspace{-0.05in}
\subsection{Algorithm Complexity}
\vspace{-0.05in}
The time complexity of training our deep multi-fidelity model is $\Ocal(N(\sum_{m=1}^M (k_ml_m)^2 + F))$ where $N$ and $F$ are the total number of training examples and NN parameters, respectively. The space complexity is $\Ocal(F + \sum_{m=1}^M (k_ml_m)^2)$, which is to store the NN parameters, and posterior mean and covariance of each random weight matrix $\W_m$. The time complexity of calculating the acquisition function is $\Ocal(\sum_{m=1}^M d_mk_m^2 + k_m^3)$. Since $k_m \ll d_m$, the complexity is linear to the output dimensions. Due to the usage of the learned variational posterior $q(\Wcal)$, the space complexity of computing the acquisition function is the same as that of training the multi-fidelity model.


==> model_copy.tex <==
%\vspace{-0.13in}
\section{Background}
%\vspace{-0.13in}
%problem definitions 
\textbf{Problem setting.}  We assume that we can query training examples with $M$ fidelities, which correspond to $M$ mappings, $\{\h_m(\x) \in \mathds{R}^{d_m}\}_{1 \le m \le M}$ where $\x \in \Xcal$ is an $r$-dimensional input, $r$ is small, $d_m$ is the output dimension, often very large, and $\{d_m\}$ are not necessarily identical.  In general, we assume $d_1 \le \ldots \le d_M$.  For instance, in structure design, the input can be  the design parameters. The high fidelity examples correspond to high-resolution structures while the low fidelity ones low-resolution structures.  We denote  by $\lambda_m$ the cost to query with fidelity $m$. Our goal is to estimate $\h_M(\x)$ (\ie the target function). Among the examples at different fidelities are strong (but complex) correlations, due to the underlying common bases, say, in physics. Hence, all these examples are valuable to estimate the target function.  To perform active learning, we begin with a small set of examples with mixed fidelities. Each step, we select both the fidelity and input location to query (or generate) new examples, so as to best balance the learning improvement (on $\h_M(\x)$) and computational cost, \ie maximizing the benefit-cost ratio. 
%Assume we can query training examples at different fidelites. Th 
%Note that this is different from popular active learning settings that assume a pool of unlabeled input examples, \eg images. Each time, we only need to rank the inputs and select the top examples to query. 
%Traditional active learning assumes a pool of unlabeled input examples, \eg images. Each time,  these examples will be ranked according to some acquisition (or utility) function computed based on the current model.  We expect the top examples will mostly improve the learning performance. We query the labels of these examples, and add them into the training set to update our model.  

\textbf{Dropout active learning.} A successful application of active learning with deep neural networks is image classification~\citep{gal2017deep,kirsch2019batchbald}. Typically, a pool of unlabeled input examples, \ie images,  is pre-collected. Each time, we rank the input examples according to an acquisition function computed based on the current model. We then query the labels of the top examples and add them into the training set. There are two popular acquisition functions. The first one is the predictive entropy of the label, 
\begin{align}
	\mathbb{H}[y|\x, \Dcal] = -\sum_{c} p(y=c|\x, \Dcal) \log p(y=c|\x, \Dcal), \label{eq:image-ac-1}
\end{align}
where $\x$ is the input, and $\Dcal$ are the training data. The other one is BALD (Bayesian active learning by disagreement)~\citep{houlsby2011bayesian}, namely the mutual information between the label and model parameters, 
\begin{align}
	\mathbb{I}[y, \btheta|\x, \Dcal]  = \mathbb{H}[y|\x, \Dcal]- \EE_{p(\btheta|\Dcal)}\left[\mathbb{H}(\y|\x, \btheta, \Dcal)\right], \label{eq:image-ac-2}
\end{align}
where $\btheta$ are the NN weights. To calculate these acquisition functions, we need to first estimate the posterior of the NN output and weights. A popular approach is to use Monte-Carlo (MC) Dropout~\citep{gal2016dropout}, which can be viewed as a variational inference method of Bayesian NNs. MC Dropout uses a probability $p_i$ to randomly drop the neurons in each layer $i$ (equivalent to zeroing out the corresponding weights) in the forward pass and performs backward pass over the remaining neurons. After training, the weights and output obtained from one such forward pass can be viewed as a sample of the approximate posterior. We can run Dropout multiple times to collect a set of posterior samples and calculate the acquisition functions by the Monte-Carlo approximation. 

\vspace{-0.05in}
\section{Deep Multi-Fidelity Modeling for High-Dimensional Outputs}
\vspace{-0.05in}
Despite its success, dropout active learning might be inappropriate for high-dimensional (continuous) outputs. When the output is a continuous vector, it is natural to use a multivariate Gaussian posterior, $p(\y|\x, \Dcal) \approx \N(\y|\bmu(\x), \bSigma(\x))$\footnote{we can also use a multivariate student $t$ distribution, but the problem remains. }, and the entropy term $\mathbb{H}(\y|\x, \Dcal)$ in the acquisition functions  (see \eqref{eq:image-ac-1} and \eqref{eq:image-ac-2}) require us to compute the log determinant of the covariance matrix, $\log|\bSigma(\x)|$. While we can use dropout samples to construct an empirical  estimate $\widehat{\bSigma}(\x)$, due to the large output dimension $n$, the computation of this $n\times n$ matrix and its log determinant is very expensive  or even infeasible. 
One might seek to only estimate the predictive variance of each individual output. However, this will ignore the strong output correlations, which is critical to effectively evaluate the uncertainty and calculate the acquisition function. Furthermore, in our active learning task, we want to optimize the acquisition function to find the best input (rather than rank the inputs in a pre-collected pool). The empirical covariance estimate from random samples can lead to numerical instability in optimization and inconsistent results from different runs. 

To overcome these problems for multi-fidelity active learning, we first propose an expressive deep multi-fidelity model, for which we develop a structural variational inference method to capture the posterior dependency of the outputs. We propose a novel acquisition function to allow multi-fidelity queries, and develop an efficient and reliable approach to calculate the acquisition function. 

Specifically, we use deep neural networks to build a multi-fidelity high-dimensional output model (see the graphical representation in Fig. 2 of the Appendix) that can flexibly, efficiently capture complex relationships between the outputs and between the fidelities, taking advantage of these relationships to enhance the learning at the highest fidelity (\ie target function).  For each fidelity $m$, we introduce a neural network (NN) that first generates a  $k_m$ dimensional  latent output, and then projects it to the $d_m$ dimensional observational space, where $k_m \ll d_m$. The NN is parameterized by $\{\W_m, \btheta_m, \A_m\}$ where $\W_m$ is a $k_m \times l_m$ weight matrix in the latent output layer, $\A_m$ a $d_m \times k_m$ projection matrix, and $\btheta_m$ the weights in all the other layers. Denote by $\x_m$ the NN input, by $\f_m(\x)$ the latent NN output, and by $\y_m(\x)$ the observation. The model is defined by
\begin{align}
&\x_m = [\x; \f_{m-1}(\x)], \;\; \f_m(\x) = \W_m\bphi_{\btheta_m}(\x_m), \notag \\
&\y_m(\x) = \A_m \f_m(\x) + \bepsilon_m, \label{eq:our-model}
\end{align}
where $\x_1 = \x$,  $\bphi_{\btheta_m}$  is the second last layer of the NN at fidelity $m$, of dimension $l_m$,\cmt{$\bphi_{\btheta_m}$ is the $l_m$ dimensional input to the output layer (hence parameterized by $\btheta_m$)} and $\bepsilon_m \sim \N(\bepsilon_m|\0, \sigma^2_m\I)$ is an isotropic Gaussian noise. Note that $\bphi_{\btheta_m}$ can be viewed as a set of nonlinear basis functions  parameterized by $\btheta_m$. Through their combinations via $\W_m$ and $\A_m$, we can flexibly capture  the complex relationships between the elements of $\y_m$ to improve the prediction. Furthermore,  the input $\x_{m}$ is constructed by appending to the original input $\x$  the latent output $\f_{m-1}$, which can be viewed as a compact  (or low-rank) summary of all the information up to fidelity $m-1$.  After a series of linear and nonlinear transformations, we obtain the latent output $\f_m$ --- the summary up to fidelity $m$ --- and then generate the high dimensional observation $\y_m$. In this way, we efficiently integrate the information from lower fidelities and capture the complex relationship between the current and previous fidelities by learning an NN mapping, $\f_m(\x) = \psi(\x, \f_{m-1}(\x))$.%, where $\psi(\cdot)$ is fulfilled by a (deep) NN. %When $m=1$, we set $\x_m = \x$. %The graphical illustration of our model is in Fig. \ref{fig:graphical}.

%Through a series of linear and nonlinear transformations inside
%the NN, we obtain the output fm(x). In this way, we digest the information from the lower fidelities,
%and capture the complex relationships between the current and previous fidelities by learning a
%nonlinear mapping fm (x) = h(x, fm−1 (x)), where h(·) is fulfilled by the NN. When m = 1, we set
%xm = x. A graphical representation of our model is given in Fig. 1 of the supplementary material.

We place a standard Gaussian prior over the elements in each $\W_m$. Similar to~\citep{snoek2015scalable}, we consider all the remaining parameters as hyper-parameters to ease the posterior inference and uncertainty reasoning. Given the training dataset $\Dcal = \{\{(\x_{nm}, \y_{nm})\}_{n=1}^{N_m}\}_{m=1}^M$, the joint probability  of our model is given by
\begin{align}
	&p(\Wcal, \Ycal|\Xcal, \Theta, \s) = \prod\nolimits_{m=1}^M \N\left(\vec(\W_m)|\0, \I\right) \notag  \\
	 &\cdot \prod\nolimits_{n=1}^{N_m} \N\big(\y_{nm}|\A_m \f_m(\x_{nm}), \sigma_m^2\I\big), \label{eq:joint-prob}
\end{align}
where $\Wcal = \{\W_m\}_{m=1}^M$,  $\Theta=\{\btheta_m, \A_m\}_{m=1}^M$, $\s = [\sigma^2_1, \ldots, \sigma^2_M]$, and $\{\Xcal$, $\Ycal\}$ are the inputs and outputs in $\Dcal$. 
To estimate the posterior of our model (which is used to calculate the acquisition function and query new examples), we develop a stochastic structural variational learning algorithm. Specifically, for each $\W_m$,  we introduce a multivariate Gaussian variational posterior, $q(\W_m) = \N\left(\vec(\W_m)|\bmu_m, \bSigma_m\right)$.  To ensure the positive definiteness, we parameterize  $\bSigma_m$ by its Cholesky decomposition, $\bSigma_m = \L_m \L_m^\top$, where $\L_m$ is a lower triangular matrix. We then assume the posterior $q(\Wcal) =\prod_{m=1}^M q(\W_m)$, and construct a variational model evidence lower bound (ELBO)~\citep{wainwright2008graphical}, $\Lcal\big(q(\Wcal), \Theta, \s\big) = \EE_{q}\left[ \log{p(\Wcal, \Ycal|\Xcal, \Theta, \s)}/{q(\Wcal)}\right] =-\text{KL}\big(q(\Wcal)\|p(\Wcal)\big) + \sum_{m=1}^M\sum_{n=1}^{N_m} \EE_q\left[\log \N(\y_{nm}|\A_m \f_m(\x_{nm}),\sigma_m^2\I)\right]$,
	% \end{align}
% \begin{align}
% &\Lcal\big(q(\Wcal), \Theta, \s\big) = \EE_{q}\left[ \log\frac{p(\Wcal, \Ycal|\Xcal, \Theta, \s)}{q(\Wcal)}\right] \notag \\
% &=-\text{KL}\big(q(\Wcal)\|p(\Wcal)\big) + \sum_{m=1}^M\sum_{n=1}^{N_m} \EE_q\left[\log \N(\y_{nm}|\A_m \f_m(\x_{nm}),\sigma_m^2\I)\right], \label{eq:elbo}
% \end{align}
where $\text{KL}(\cdot \| \cdot)$ is Kullback Leibler divergence and $p(\Wcal)$ the prior of $\Wcal$. We maximize $\Lcal$ to jointly estimate $q(\Wcal)$ and the hyper-parameters. While $\Lcal$ is intractable, it is straightforward to use the reparameterization trick~\citep{kingma2013auto} to generate parameterized samples for each $\vec(\W_m)$: $\bmu_m + \L_m \bxi_m$ where $\bxi_m \sim \N(\0, \I)$ to obtain a stochastic estimate of $\Lcal$,  and perform efficient stochastic optimization. %We left the details in the supplementary material. 
 
 %multi-fidelit queries
 %\vspace{-0.1in}
\section{Multi-Fidelity Active Learning}
%\vspace{-0.1in}
\subsection{Mutual Information based Acquisition Function}
%\vspace{-0.1in}
We now consider how to perform active learning with multi-fidelity queries. We assume that at each fidelity $m$, the most valuable training example is the one that can best improve our prediction of the target function, namely, the prediction at the highest fidelity $M$. 
To this end, we propose our acquisition function based on the mutual information between the outputs at fidelity $m$ and $M$,
\begin{align}
	&a(\x, m)  = \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x)  \y_M(\x)|\Dcal\right) \notag \\
	&= \frac{1}{\lambda_m} \big(\mathbb{H}(\y_m|\Dcal) +\mathbb{H}(\y_M|\Dcal) - \mathbb{H}(\y_m, \y_M|\Dcal) \big), \label{eq:ac}
\end{align}
%\begin{align}
%	a(\x, m)  &= \frac{1}{\lambda_m} \mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right), \notag \\
%	&= \frac{1}{\lambda_m} \left(\mathbb{H}(\y_m(\x)|\Dcal) +\mathbb{H}(\y_M(\x)|\Dcal) - \mathbb{H}(\y_m(\x), \y_M(\x)|\Dcal) \right) \label{eq:ac}
%\end{align}
where $\lambda_m>0$ is the cost of querying a training example with fidelity $m$. When $m=M$, we have $a(\x, M) = \frac{1}{\lambda_M} \mathbb{H}\left(\y_M(\x)|\Dcal\right)$ ---  the output entropy.  Therefore, our acquisition function is an extension of the popular predictive entropy principle in conventional active learning.  At each step, we maximize our acquisition function to identify a pair of fidelity and input location that give the biggest benefit-cost ratio.  %Note that we can also adjust the BALD principle [??] in the multi-fidelity setting,  $a_{\text{BALD}} = \frac{1}{\lambda_m}$ However, given all the parameters, the uncertainty of the output only comes form the Gaussian noise, ....

%talk about BALD

%challengen, our method
%\vspace{-0.1in}
\subsection{Efficient Acquisition Function Calculation}\label{sect:ac-compute}
%\vspace{-0.1in}
To maximize the acquisition function \eqref{eq:ac}, a critical challenge is to compute the posterior of the outputs $\{\y_m\}$ in every fidelity, based on our model estimation results, \ie $p(\Wcal|\Dcal) \approx q(\Wcal)$.  Due to the high dimensionality of each $\y_m$ and the nonlinear coupling of the latent outputs across the fidelities (see \eqref{eq:our-model}), the computation is challenging and analytically intractable.  To address this issue, we consider approximating the posterior of the low dimensional latent output $\f_m$ first, which can be viewed as a function of the random NN weights $\bOmega_m = \{\W_1, \ldots, \W_m\}$ (given the input $\x$). We then use multivariate delta method~\citep{oehlert1992note,bickel2015mathematical} to compute the moments of $\f_m$. Specifically, we approximate $\f_m$ with a first-order Taylor expansion, 
\begin{align}
	\f_m(\bOmega_m) \approx \f_m(\EE[\bOmega_m]) + \J_m\left(\boldeta_m  - \EE[\boldeta_m]\right), \label{eq:1order}
\end{align}
where the expectation is under $q(\cdot)$,  $\boldeta_m = \vec(\bOmega_m)$, $\J_m = \frac{\partial \f_m}{\partial \boldeta_m}|_{\boldeta_m = \EE[\boldeta_m]}$ is the Jacobian matrix at the mean.  The rationale is as follows. First, $\f_m$ is linear to $\W_m$ and the second-order derivative is simply $\0$.  Second, as the NN output, $\f_m$ is highly nonlinear to the random weights in the previous  layers,  $\W_j$ ($j<m$). Hence, we can assume the change rate of $\f_m$ (gradient or Jacobian) has much greater scales than the posterior covariance of $\W_j$ in the second-order term of the Taylor expansion. Note that $q(\W_j)$ is much more informative and hence much more concentrated than the prior $ \N(\vec(\W_j)|\0, \I)$. The scale of the posterior covariance should be much smaller than $1$. Integrating both cases, the first-order term can dominate the Taylor expansion and hence we ignore the higher order terms. 
Based on \eqref{eq:1order}, we can easily calculate the first and second moments of $\f_m$, 
\begin{align}
	\balpha_m &= \EE[\f_m] \approx \f_m\left(\EE[\bOmega_m]\right), 	\\
	 \V_m &= \text{cov}[\f_m] \approx \J_m \text{cov}(\boldeta_m) \J_m^\top, 
\end{align}
where  $\text{cov}(\boldeta_m) = \diag\left(\left\{\text{cov}\big(\vec(\W_j)\big)\right\}_{1\le j\le m}\right)$. 
Then we use moment matching to estimate a joint Gaussian posterior, $q(\f_m)  = \N(\f_m|\balpha_m, \V_m)$. Next, according to \eqref{eq:our-model}, we can obtain the posterior of the output $\y_m$, 
\begin{align}
	q(\y_m) = \N(\y_m|\A_m \balpha_m, \A_m \V_m \A_m^\top + \sigma_m^2\I).
\end{align}
The output entropy is  $\mathbb{H}(\y_m|\Dcal) = \frac{1}{2}\log|\A_m \V_m \A_m^\top + \sigma_m^2\I| + d_m \log\sqrt{2\pi e}$.  However, directly computing the log determinant of a $d_m \times d_m$ matrix is very expensive. We further use the Weinstein-Aronszajn identity~\citep{kato2013perturbation} to derive 
\begin{align}
	&\mathbb{H}(\y_m|\Dcal) =  \frac{1}{2}\log|\sigma_m^{-2}\A_m \V_m \A_m^\top + \I|  + d_m \log \sqrt{2\pi e\sigma_m^2} \notag \\
	&=\frac{1}{2}\log|\sigma_m^{-2}\A_m^\top\A_m\V_m + \I| + d_m \log \sqrt{2\pi e\sigma_m^2}. \label{eq:en_ym}
\end{align}
Now, the log determinant is calculated on a much smaller, $k_m \times k_m$ matrix, which is very cheap and efficient. 

Using a similar approach, we can calculate the joint posterior of $\barf_m = [\f_m; \f_M]$ and then $\bary_m=[\y_m; \y_M]$.  First, we view $\barf_m$ as a function of all the random weights, $\Wcal = \{\W_1, \ldots, \W_M\}$. We use the multivariate delta method and moment matching to estimate a joint Gaussian posterior, 
$q(\barf_m) = \N(\barf_m|\baralpha_m, \barV_m)$ where $\baralpha_m = \barf_m\left(\EE[\Wcal]\right)$,  $\barV_m = \barJ_m \text{cov}(\boldeta)\barJ_m^\top$, $\boldeta = \vec(\Wcal)$, $\barJ_m = \frac{\partial \barf_m}{\partial \boldeta}|_{\boldeta = \EE[\boldeta]}$, and $\text{cov}(\boldeta) = \diag\left(\left\{\text{cov}\big(\vec(\W_j)\big)\right\}_{1\le j\le M}\right)$. According to our model \eqref{eq:our-model}, we can represent
\[
\bary_m = \barA_m \barf_m + \bareps_m,
\]
where $\barA_m = \diag(\A_m, \A_M)$ and $\bareps_m = [\bepsilon_m; \bepsilon_M]$. Therefore, the joint posterior of $\bary_m$ is 
\begin{align}
	q(\bary_m) = \N(\bary_m|\barA_m \baralpha_m, \barA_m \barV_m \barA_m^\top + \S_m),
\end{align}
where $\S_m = \diag(\sigma^2_m\I_{d_m}, \sigma^2_M \I_{d_M})$,  $\I_{d_m}$ and $\I_{d_M}$ are identity matrices of $d_m \times d_m$ and $d_M \times d_M$, respectively.  Again, we use  Weinstein-Aronszajn identity to simplify the entropy computation of $\bary_m$ (\ie $\y_m$ and $\y_M$), 
\begin{align}
	&\mathbb{H}(\y_m, \y_M|\Dcal)  =\frac{1}{2}\log|\S_m^{-1}\barA_m \barV_m \barA_m^\top + \I|  + \xi_m \notag \\
	&=\frac{1}{2}\log|\barA_m^\top \S_m^{-1} \barA_m \barV_m + \I| + \xi_m, \label{eq:en_ymM}
\end{align}
where $\xi_m = d_m \log \sqrt{2\pi e\sigma_m^2} + d_M \log \sqrt{2\pi e\sigma_M^2}$ and the log determinant is computed from a $(k_m + k_M) \times (k_m + k_M)$ matrix, which is cheap and efficient. Note that we can use matrix blocks to compute $\barA_m^\top \S_m^{-1} \barA_m = \diag\left(\sigma_m^{-2}\A_m^\top \A_m, \sigma_M^{-2}\A_M^\top \A_M\right)$.

Now, based on \eqref{eq:en_ym} and \eqref{eq:en_ymM}, we can calculate our acquisition function \eqref{eq:ac} in an analytic and deterministic way. For each fidelity $m$, we maximize $a(\x, m)$ w.r.t to $\x$ to find the optimal input. We can use automatic differential libraries to calculate the gradient and feed it to any optimization algorithm, \eg L-BFGS.   We then use the optimal input at the fidelity that has the largest acquisition function value to query  the next training example. Our deep multi-fidelity active learning is summarized in Algorithm \ref{alg:dmf-al}. 
%problem of dropout ... 
\setlength{\textfloatsep}{20pt}
\begin{algorithm}                      % enter the algorithm environment
	\small
	\caption{\ours($\Dcal$, $T$, $\{\lambda_m\}_{m=1}^M$ )}          
	\label{alg:dmf-al}                           
	\begin{algorithmic}[1]                    % enter the algorithmic environment
		\STATE Train the deep multi-fidelity model \eqref{eq:joint-prob} on the initial dataset $\Dcal$ with stochastic structural variational learning.  
		\FOR {$t=1,\ldots, T$}
		\STATE Based on \eqref{eq:en_ym} and \eqref{eq:en_ymM}, calculate and optimize the acquisition function \eqref{eq:ac} to find 
		\begin{align}
			(\x_{t}, m_{t}) = \argmax_{\x \in \Xcal, 1\le m \le M} a(\x, m).\notag % =  \frac{1}{\lambda_m}\mathbb{I}\left(\y_m(\x), \y_M(\x)|\Dcal\right).\notag
		\end{align}
		\STATE Query the output $\y_{t}$ at input $\x_t$ with fidelity $m_t$. %(\eg running a numerical solver).
		\STATE $\Dcal \leftarrow \Dcal \cup \{(\x_{t}, \y_{t})|m_t\}$.
		\STATE Re-train the deep multi-fidelity model on $\Dcal$.
		\ENDFOR
		%\vspace{-0.05in}
		%\RETURN the current posterior $q_{cur}(\cdot)$.
	\end{algorithmic}
\end{algorithm}
 %\setlength{\floatsep}{5pt}
 \vspace{-0.05in}
\subsection{Algorithm Complexity}
\vspace{-0.1in}
The time complexity of training our deep multi-fidelity model is $\Ocal(N(\sum_{m=1}^M (k_ml_m)^2 + F))$ where $N$ and $F$ are the total number of training examples and NN parameters, respectively. The space complexity is $\Ocal(F + \sum_{m=1}^M (k_ml_m)^2)$, which is to store the NN parameters, and posterior mean and covariance of each random weight matrix $\W_m$. The time complexity of calculating the acquisition function is $\Ocal(\sum_{m=1}^M d_mk_m^2 + k_m^3)$. Since $k_m \ll d_m$, the complexity is linear in the output dimensions. Due to the usage of the learned variational posterior $q(\Wcal)$, the space complexity of computing the acquisition function is the same as that of training the multi-fidelity model.

